ConvBKI: Real-Time Probabilistic Semantic Mapping Network with Quantifiable Uncertainty

In this paper, we develop a modular neural network for real-time {\color{black}(> 10 Hz)} semantic mapping in uncertain environments, which explicitly updates per-voxel probabilistic distributions within a neural network layer. Our approach combines the reliability of classical probabilistic algorithms with the performance and efficiency of modern neural networks. Although robotic perception is often divided between modern differentiable methods and classical explicit methods, a union of both is necessary for real-time and trustworthy performance. We introduce a novel Convolutional Bayesian Kernel Inference (ConvBKI) layer which incorporates semantic segmentation predictions online into a 3D map through a depthwise convolution layer by leveraging conjugate priors. We compare ConvBKI against state-of-the-art deep learning approaches and probabilistic algorithms for mapping to evaluate reliability and performance. We also create a Robot Operating System (ROS) package of ConvBKI and test it on real-world perceptually challenging off-road driving data.

==> DynamicMapping.tex <==
% Introduce the layer
% Demonstrate results
% What is the issue with the layer?
\section{Dynamic Mapping}\label{sec:DynamicMapping}
Although the proposed algorithm is capable of integrating semantic predictions into a map in real-time, it is still vulnerable to dynamic objects. As objects move, they violate the static assumption implicit in our method and leave smears \cite{DynamicBKI}. In this section we propose a deformable geometric attention layer which explicitly propagates concentration parameters of dynamic objects in a real-time, differentiable layer. 

\jw{Many citations here}
\subsection{Dynamic Objects} 
Dynamic objects can corrupt data sets \cite{SemanticKITTI, MotionSC} and algorithms \cite{MappingSBKI} alike. There are several existing methods to handle dynamic objects including segmenting foreground from background, post-rejection of dynamic objects after map creation, or integrating dynamic objects within the map. Segmenting foreground from background allows the robot to discard points corresponding to dynamic classes and separately track dynamic objects. However, this method is inefficient as it requires two separate world models. Post-rejection of dynamic objects similarly leads to an un-representative world model. 

Algorithms which propose to integrate dynamic objects within a world model may be divided into two classes: probabilistic algorithms and networks operating in a latent space. Probabilistic methods are hand-crafted and mathematical which leads to trustworthiness and reliability as equations may transfer between data sets, however they are generally slow and not optimized as they do not take advantage of breakthroughs in deep learning. Deep neural networks are able to efficiently handle dynamic objects in a single unified framework through mechanisms such as attention, however they typically operate in a latent space and fail to transfer to new data \cite{MotionSC}. A recent work proposed to combine probabilistic methods with deep learning by leveraging velocity estimates from scene flow networks as input to a world model which exponentially decays traces left by dynamic objects \cite{DynamicBKI}. However, the approach failed to consider a propagation step and only decayed belief that an object remained in the same location. Therefore, we propose a novel attention method which combines probabilistic methods with deep learning to propagate dynamic objects within a single world model. 

Attention is a deep learning mechanism which learns to weight incoming data or features in a normalized sum. Attention layers can be combined to form transformers, which have revolutionized fields such as natural language processing. Transformers can be improved through deformable attention, which allows the network to learn an offset over a spatial grid before performing a normalized sum. 

\begin{figure}[t]
    \includegraphics[width=0.5\linewidth]{Images/DeformableAttention.png}
    \centering
    \caption{Illustration of deformable geometric attention layer. The inputs to the layer are deformable offsets and probabilities, which may be directly interpreted as the negative of motion and object classification probability. 
    }
    \label{fig:DeformableAttention}
    \vspace{-4mm}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{Images/BKINet.png}
    \caption{Overview of BKINet. The input is any form of 3D data $X_t$, and pose XX. Static concentration parameters of the local map from the previous time step, $L_{t-1}$, are moved to pose XX through the local transform module. The object tracking network predicts classification scores and offsets for each voxel, which are used to propagate concentration parameters of dynamic objects in the deformable geometric attention layer. Finally, semantic segmentation labels are predicted for all incoming data and input to a ConvBKI layer which updates the local map. The process repeats as new data is obtained. \jw{Add example point cloud to the left, and example map to the right}}
    \label{fig:bkinet}
\end{figure*}

\jw{Math equations required}
\subsection{Deformable Geometric Attention}
Our layer is composed of two steps. First, a network performs object detection and estimates offsets for each object. Second, concentration parameters from the map prior are translated to their new positions with weights learned from geometric attention and object detection. For voxel $*$, 

\begin{equation}
    \bar{\alpha}^c_{*, t} = p_* \: \text{interp}(x_* + o_{t-1:t}, \hat{L}_t) \; \forall c \; \in \mathcal{D}
\end{equation}

where $x_*$ is the centroid of voxel $*$ with offset $o_{t-1:t}$, classification probability $p_*$, and channel $c$ in the set of dynamic categories $\mathcal{D}$.  

Exteroceptive sensor data from the current and previous frames is provided to an object tracking network which predicts a probability for each voxel in the local map, and a deformable offset. We use MotionNet \cite{MotionNet} due to its lightweight architecture and low latency, however any object tracking network is a suitable substitute. The deformable offset $o_{t-1:t} \in R(3)$ provides a sampling offset from the current local map to the previous local map. Note that the offset is an estimation from $t$ to $t-1$, instead of a prediction of movement from $t-1$ to $t$. Rearranging the terms allows for improved tracking, and efficient grid sampling. The probability score for each voxel indicates whether a dynamic class, eg. human or car, is present at a voxel, regardless of whether the object is moving or not. The probability provides a weight to edges established by the deformable offset. 

Next, concentration parameters for dynamic classes are re-sampled with edges established by the deformable offset of each voxel, and weights of the classification score. An illustration of the update is shown in Figure \ref{fig:DeformableAttention}. For each voxel in the new local map, static and dynamic classes are updated separately. Since static classes do not move, there is no special update procedure. Dynamic classes, however, lead to dependencies upon different locations from the previous local map. For each voxel, the dependency to a different spatial location is modeled by a deformable offset. The deformable offset informs the world model on which spatial locations from the previous map correspond to new locations in the regular voxel grid of the current frame. Concentration parameters for dynamic classes at each voxel are then calculated by tri-linear interpolation from the offset locations of the previous local map. Note that while sampling weights may be learned, tri-linear interpolation provides an efficient, differentiable, and mathematical solution to sampling from a grid with explicit parameters. 

However, several problems arise from the proposed deformable sampling method. Edges are established at every voxel regardless of whether a dynamic object is present, and the concentration parameters do not decay, indicating a constant or increasing certainty. Therefore, the classification score provides a method to increase uncertainty and remove edges.  

% \begin{itemize}
%     \item Success of attention, deformable attention elsewhere. 
%     \item Geometric interpretation: offset of dynamic object. Figure.
%     \item Formal definition. Input: offsets and probability. Probability [0 to 1] used to scale, since require forward correspondence or the same object may appear at multiple locations. 
% \end{itemize}

% The goal of the layer is to propagate dynamic concentration parameters from the previous timestep to the current timestep. While directly translating voxel centroids to the next frame would be convenient, there is no efficient solution as the transformed voxels do not align along a grid. Instead, it is more convenient to sample the voxels of the current map by an offset from their centroid, generating sampling locations from the previous map. This operation may be directly interpreted as deformable attention, since attention refers to a normalized sum, and deformable refers to the offset. The offset in this case is a 3D vector opposite the motion of the object, indicating which voxel is now in the current location. Since sampling is performed in continuous space on a grid, the normalized sum may be replaced with tri-linear interpolation to approximate concentration parameters. 

% One challenge, however, emerges when transforming centroids from the current time step. A sense of forward correspondence is lost, where the same voxel from previous frames may be sampled multiple times. For example, offsets may point to the same location. The voxel a car moved from may sample itself, resulting in the vehicle appearing both static and as if it had moved. Therefore, a probability vector is also necessary to enable forward correspondence by assigning zero weight to unoccupied voxels. Concretely, the input is a 3D offset per voxel and 1D probability $\in [0, 1]$, with attention weights calculated by tri-linear interpolation. Sampled concentration parameters for dynamic classes are multiplied by the probability vector, which has an additional bonus of increasing variance. 

% In practice, these labels may be easily computed by any object detection algorithm. We choose MotionNet, since it runs in real-time and is easy to train. MotionNet is modified to predict a 3D translation vector from the current time step to the previous time step (deformable offset) and a classification probability. 

